Iterative Spectral Method for Alternative Clustering

Given a dataset and an existing clustering as input, alternative clustering aims to find an alternative partition. One of the state-of-the-art approaches is Kernel Dimension Alternative Clustering (KDAC). We propose a novel Iterative Spectral Method (ISM) that greatly improves the scalability of KDAC. Our algorithm is intuitive, relies on easily implementable spectral decompositions, and comes with theoretical guarantees. Its computation time improves upon existing implementations of KDAC by as much as 5 orders of magnitude.

==> section_4A_Scalability.tex <==
\section{Scalability}\label{sec:scalability}
\chieh{The scalability adventage of ISM is two folds. First, the most computational complex portion of the algorithm is the eigen decomposition of $\Phi(W) \in \mathbb{R}^{d \times d}$. Since $d<<N$, the scalability is decoupled from the size of the data. Even if high dimensional data is used, the eigendecomposition within ISM only requires q eigenvectors. Since $q << N$, there exist many techniques to approximate eigenvectors, e.g, the power method. There also exist off the shelf GPU implementations of eigendecomposition (MAGMA, cuBLAS). To further improve the speed, updates of U can also be improved via the Variational Nystrom method, Vladymyrov et al. ICML16. Our key contribution is to provide theoretical guarantees for the spectral method to leverage existing research and technology. Second,   the proposed initialization is intimately tied to the ISM method. It results from applying the 2nd order Taylor approximation to the objective to approximate a closed form solution of the global minimum. Having a starting point close to the global minimum simultaneously improves convergence rate and the quality of the solution.}


